Quality In / Quality Out: Data quality more relevant than model choice in anomaly detection with the UGR'16

Autonomous or self-driving networks are expected to provide a solution to the myriad of extremely demanding new applications with minimal human supervision. For this purpose, the community relies on the development of new Machine Learning (ML) models and techniques. %, like the celebrated Deep Learning (DL). However, ML can only be as good as the data it is fitted with, and data quality is an elusive concept difficult to assess. In this paper, we show that relatively minor modifications on a benchmark dataset (UGR'16, a flow-based real-traffic dataset for anomaly detection) cause significantly more impact on model performance than the specific ML technique considered. We also show that the measured model performance is uncertain, as a result of labelling inaccuracies. Our findings illustrate that the widely adopted approach of comparing a set of models in terms of performance results (e.g., in terms of accuracy or ROC curves) may lead to incorrect conclusions when done without a proper understanding of dataset biases and sensitivity. We contribute a methodology to interpret a model response that can be useful for this understanding.

==> 2.Related.tex <==
One of the key steps in the ML pipeline is data preparation. The process of transforming raw data into features has a huge impact on ML performance. Feature extraction can be performed using linear and nonlinear methods %such as Principal Component Analysis (PCA), Partial Least Squares regression (PLS), Linear discriminant analysis (LDA), Independent Component Analysis (ICA), Multi-Dimensional Scaling (MDS), Fourier transform, kernel-based PCA, manifold learning algorithms, k-means, neural networks, and others 
\cite{Jia2022}\cite{LeonMedina2020}\cite{Piernik2021}\cite{ Horii2021}. Parsing is also a popular method \cite{Kiran2019}. 
Feature selection often provides better predictive power and optimizes the dimensions of the feature space, thus reducing complexity \cite{Benkessirat2019}\cite{Jovic2015}. %Many methods are used in this part of data preparation: correlation analysis, ANOVA, Chi-square test, Fisher score, Causal Bayesian Networks, Markov Blanket Induction \cite{Benkessirat2019}\cite{Jovic2015}, as well as Multilayer Perceptrons \cite{Romero2008}), Self-Organizing Maps (SOM) \cite{Silva2021}, Genetic Programming \cite{Cava2017}, Reinforcement Learning \cite{Zhang2019}, and others.

Due to the various methods of collecting and preparing datasets, and the problems associated with these processes (for example, device or human errors), it is necessary to assess the quality of the dataset before ML modeling. While there is no formal definition of the quality of a dataset, we can say that the quality of a dataset is the degree to which a dataset fulfills the requirements for its intended use. Data quality is typically referred to the multi-dimensional concept \cite{Wang1996}. In order to determine the quality of the data, the following dimensions have been proposed: accuracy, completeness, validity, timeliness, consistency, correctness, uniqueness, reliability, and others. These indicators help understand the data, but while intuitive, they are difficult to measure in practice \cite{Li2012} \cite{Heinrich2018}. The meaning and importance of each dimension and its metric varies from application to application \cite{Sidi2012}. Several of these indicators have been adapted in the networking area, but there is no framework to assist in assessing each network dataset \cite{Verma2019}. Yet, the assessment of data quality should be a priority for the network community, as a recent survey on intrusion datasets points out \cite{kenyon_are_2020}.

%Given the complexity associated to assessing data quality, most literature focus on the improvement of the modelling step. To improve model performance, dataset cleaning is usually performed. Data cleaning is the process of detecting and correcting/removing corrupted or inaccurate observations from a dataset \cite{Sammut2017}. This process only allows us to get rid of common problems, such as missing values, duplicates, outliers, or class imbalance. The influence of the order of cleaning operations on the effect of cleaning dataset was analyzed in \cite{Cheng2018}. However, there exist additional problems that are often ignored, such as class overlapping or mislabeling \cite{camacho2022dataset}. These problems affect the data quality and, thus, the resulting model built from them. 
%In addition, the cleaning operation may improve some indicator mentioned above, but it may affect another indicator \cite{Fan2014}. 
 
The research on data quality is gaining momentum in the community. The influence on model performance of data normalization and dimensionality reduction is studied in \cite{obaid2019impact}. Gonzalez \cite{gonzalez_zelaya_towards_2019} proposes a method to assess the influence of specific steps on data preparation on model performance. In this work we are not so interested on establishing preprocessing effects on model quality that can be generalized to other datasets: our findings are very specific of the dataset under study, but the fact that minor preprocessing steps affect model performance is a useful message for the community.  

There is an inherent connection of data quality and labelling. The relevance and challenges of labelling in network traffic datasets are emphasized in \cite{guerra_datasets_2022}. Landauer et al. \cite{landauer2022framework} introduce a framework for automatic labelling of datasets to train host intrusion detection systems.  Camacho and Wasielewska \cite{camacho2022dataset} introduce a method of labels permutation in order to estimate the quality of association of a dataset with a specific labelling. Our findings in this paper support the need to study the quality of labelling in network datasets, which of specially relevance given that a wrong labelling can detriment our perception of model quality and thus the potential conclusions derived from the study. In connection to this limitation, Laur\'ia and Tayi \cite{lauria_comparative_nodate} and Chen et al. \cite{chen_data_2021} perform similar studies to the present one, evaluating the influence of data quality in model performance. These works, however, perform a more coarse analysis, and assume that the labelling of the datasets is correctly. Our work introduces a methodology to perform a deep analysis to get a full understanding on how data characteristics affect model performance, which can lead to identify labelling errors.    


In our article, we compare the influence on anomaly detection performance in a benchmark dataset of the data preprocessing/selection and the ML technique choice. To the best of our knowledge, this is the first time that such experiment is performed. 

